FlowEval: A Consensus-Based Dialogue Evaluation Framework Using Segment Act Flows

Despite recent progress in open-domain dialogue evaluation, how to develop automatic metrics remains an open problem. We explore the potential of dialogue evaluation featuring dialog act information, which was hardly explicitly modeled in previous methods. However, defined at the utterance level in general, dialog act is of coarse granularity, as an utterance can contain multiple segments possessing different functions. Hence, we propose segment act, an extension of dialog act from utterance level to segment level, and crowdsource a large-scale dataset for it. To utilize segment act flows, sequences of segment acts, for evaluation, we develop the first consensus-based dialogue evaluation framework, FlowEval. This framework provides a reference-free approach for dialog evaluation by finding pseudo-references. Extensive experiments against strong baselines on three benchmark datasets demonstrate the effectiveness and other desirable characteristics of our FlowEval, pointing out a potential path for better dialogue evaluation.

==> table/intent_distribution.tex <==
\begin{table*}[t!]
  \centering
  \small
  \begin{tabular}{p{0.15\textwidth}lcc|ccc}
    \toprule
    & & \multicolumn{2}{c|}{\textbf{ConvAI2}} &\multicolumn{3}{c}{\textbf{DailyDialog}} \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-7} 
    & & Train set & Validation Set & Train set & Validation Set & Test set \\
    \midrule
    \multirow{4}{*}{General Task} & \textsl{inform} & 0.69474 & 0.72971 & 0.61322 & 0.55424 & 0.60376 \\
    & \textsl{question} & 0.16303 & 0.16195 & 0.16368 & 0.16964 & 0.16440 \\
    & \textsl{directive} & 0.01180 & 0.01286 & 0.06783 & 0.08564 & 0.07169 \\
    & \textsl{commissive} & 0.00083 & 0.00144 & 0.01325 & 0.03382 & 0.01254 \\
    \midrule
    \multirow{4}{0.15\textwidth}{Social Obligation Management} & \textsl{greeting} & 0.05852 & 0.03431 & 0.02188 & 0.02994 & 0.02221 \\
    & \textsl{goodbye} & 0.00043 & 0.00123 & 0.00499 & 0.00545 & 0.00374 \\
    & \textsl{apology} & 0.00430 & 0.00356 & 0.00794 & 0.00939 & 0.01042 \\
    & \textsl{thanking} & 0.00524 & 0.00568 & 0.02339 & 0.03085 & 0.02390 \\
    \midrule
    \multirow{3}{*}{Simple Feedback} & \textsl{backchannel-success} & 0.06088 & 0.04871 & 0.08307 & 0.08036 & 0.08504 \\
    & \textsl{backchannel-failure} & 0.00017 & 0.00041 & 0.00050 & 0.00055 & 0.00143 \\
    & \textsl{check-understanding} & 0.00006 & 0.00014 & 0.00026 & 0.00012 & 0.00087 \\
    \bottomrule
  \end{tabular}
  \caption{\label{tab:intent-dist}
  Communicative intent distribution on ConvAI2 and DailyDialog.
  }
\end{table*}


==> table/intent_example.tex <==
\begin{table*}[t!]
  \centering
  \small
  \begin{tabular}{lllr}
    \toprule
    \multicolumn{1}{l}{\bf General Dimension} & \multicolumn{1}{c}{\bf Segment Act} & \multicolumn{1}{c}{\bf Example} & 
    \multicolumn{1}{r}{\bf Distribution} \\
    \midrule 
    \multirow{4}{0.2\textwidth}{General Task} & \texttt{question} & ``What time is it?'' & 67.077\% \\
    & \texttt{inform} & ``The train is leaving.'' & 16.333\% \\
    & \texttt{directive} & ``Please don’t do this ever again.'' & 2.871\% \\
    & \texttt{commissive} & ``I will not do that any more.'' & 0.494\% \\
    \midrule
    \multirow{4}{0.2\textwidth}{Social Obligation Management} & \texttt{greeting} & ``how are you?'', ``I'm fine.'' & 4.702\% \\
    & \texttt{goodbye} & ``Bye'', ``see you.'' & 0.178\% \\
    & \texttt{apology} & ``Sorry.'', ``No problem.'' & 0.542\% \\
    & \texttt{thanking} & ``Thanks.'', ``You are welcome.'' & 1.074\% \\
    \midrule
    \multirow{3}{0.2\textwidth}{Simple Feedback} & \texttt{backchannel-success} & ``Okay'', ``Uh-huh'' & 6.686\% \\
    & \texttt{backchannel-failure} & ``Sorry?'', ``Excuse me?'' & 0.030\% \\
    & \texttt{check-understanding} & ``Do you get what I just said?'' & 0.013\% \\
    \bottomrule
  \end{tabular}
  \caption{\label{table:intent-example}
  Examples and distribution of \dataset{}, our segment act dataset.}
\end{table*}

